Best-of-N Jailbreaking

We introduce Best-of-N (BoN) Jailbreaking, a simple black-box algorithm that jailbreaks frontier AI systems across modalities. BoN Jailbreaking works by repeatedly sampling variations of a prompt with a combination of augmentations - such as random shuffling or capitalization for textual prompts - until a harmful response is elicited. We find that BoN Jailbreaking achieves high attack success rates (ASRs) on closed-source language models, such as 89% on GPT-4o and 78% on Claude 3.5 Sonnet when sampling 10,000 augmented prompts. Further, it is similarly effective at circumventing state-of-the-art open-source defenses like circuit breakers. BoN also seamlessly extends to other modalities: it jailbreaks vision language models (VLMs) such as GPT-4o and audio language models (ALMs) like Gemini 1.5 Pro, using modality-specific augmentations. BoN reliably improves when we sample more augmented prompts. Across all modalities, ASR, as a function of the number of samples (N), empirically follows power-law-like behavior for many orders of magnitude. BoN Jailbreaking can also be composed with other black-box algorithms for even more effective attacks - combining BoN with an optimized prefix attack achieves up to a 35% increase in ASR. Overall, our work indicates that, despite their capability, language models are sensitive to seemingly innocuous changes to inputs, which attackers can exploit across modalities.

==> analytical_errors_vs_bootstrapping.tex <==
\section{Statistical Analysis of Error Estimation}
\label{app:maths_bootstrap}

We develop a statistical framework to analyze the uncertainty in Best-of-N (BoN) jailbreaking across two key dimensions: the uncertainty in estimating the probability of success for each individual request, and the variability in observed trajectories given these probabilities.

\paragraph{Model Setup} For each request $i$, we model the number of trials until successful jailbreak ($n_i$) as following a geometric distribution truncated at the maximum number of trials $N$. Let $p_i$ be the true probability of success for request $i$. Then the probability mass function is:

\begin{equation}
    P(n_i = k|p_i) = \begin{cases}
        p_i(1-p_i)^{k-1} & \text{if } k < N \\
        (1-p_i)^{N-1} & \text{if } k = N
    \end{cases}
\end{equation}

\paragraph{Maximum Likelihood Estimation and Bias} The MLE for uncensored observations ($n_i < N$) is $\hat{p}_{i,MLE} = \frac{1}{n_i}$. This estimator is upward-biased due to Jensen's inequality and the convexity of the reciprocal function:

\begin{equation}
    E[\frac{1}{n_i}] > \frac{1}{E[n_i]} = p_i
\end{equation}

The magnitude of this bias can be computed exactly for the geometric distribution:

\begin{equation}
    E[\frac{1}{n_i}] = p_i \sum_{k=1}^{\infty} \frac{1}{k}(1-p_i)^{k-1} = \frac{-p_i}{(1-p_i)}\ln(p_i)
\end{equation}

This bias is particularly severe for small values of $p_i$, where the relative error can exceed 100\%.

\paragraph{Bayesian Estimation} We adopt a Bayesian approach with a log-uniform prior $P(p_i) \propto \frac{1}{p_i}$, yielding for uncensored observations the bias-corrected estimator:

\begin{equation}
    \hat{p}_i = \frac{1}{n_i + 1}
\end{equation}

For censored observations ($n_i = N$), rather than using the point estimate $\frac{1}{N + 1}$, we sample from the posterior distribution:

\begin{equation}
    p_i|n_i=N \sim \text{Beta}(1, N)
\end{equation}

This better represents our uncertainty about these censored probabilities while respecting the constraint that $p_i < \frac{1}{N}$.

\paragraph{Error Curves} The expected ASR at step $k$ is:

\begin{equation}
    E[\text{ASR}(k)] = \frac{1}{R}\sum_{i=1}^R (1-(1-\hat{p}_i)^k)
\end{equation}

The variance at each step $k$ has two components. First, the binomial variance given fixed probabilities:

\begin{equation}
    \text{Var}_1(k) = \frac{1}{R^2}\sum_{i=1}^R (1-(1-\hat{p}_i)^k)(1-\hat{p}_i)^k
\end{equation}

Second, the variance due to uncertainty in our probability estimates:

\begin{equation}
    \text{Var}_2(k) = \frac{1}{R^2}\sum_{i=1}^R k^2(1-\hat{p}_i)^{2k-2}\text{Var}(\hat{p}_i)
\end{equation}

The total standard deviation curves are then:

\begin{equation}
    \sigma(k) = \sqrt{\text{Var}_1(k) + \text{Var}_2(k)}
\end{equation}

These curves form envelopes around the expected ASR curve, with width:

\begin{equation}
    E[\text{ASR}(k)] \pm \sigma(k)
\end{equation}

\paragraph{Characteristic Shape} The error curves have several notable properties:
\begin{itemize}
    \item The variance is zero at $k=0$ (ASR always 0)
    \item The variance peaks in the mid-range of $k$ where some but not all requests have succeeded
    \item The variance decreases as $k \to \infty$ as all requests with $p_i > 0$ eventually succeed
    \item For censored observations, the uncertainty from sampling posterior probabilities creates a persistent variance even at large $k$
\end{itemize}

The error envelope is asymmetric due to the bounded nature of ASR (between 0 and 1), with larger upward variance when ASR is low and larger downward variance when ASR is high. This asymmetry can be captured more accurately using beta distribution approximations rather than normal approximations for the confidence intervals.

\paragraph{Combined Analysis} Incorporating both the bias-corrected estimators for uncensored observations and sampled probabilities for censored ones, we can compute the full uncertainty in our ASR estimates. For a given confidence level $\alpha$, we construct confidence intervals as:

\begin{equation}
    \text{CI}_{\alpha}(k) = E[\text{ASR}(k)] \pm z_{\alpha/2}\sigma(k)
\end{equation}

where $z_{\alpha/2}$ is the appropriate quantile of the standard normal distribution. For more accurate intervals that respect the [0,1] bounds of ASR, we can use the beta distribution approximation:

\begin{equation}
    \text{CI}_{\alpha}(k) = \text{Beta}^{-1}(\alpha/2, \alpha_k, \beta_k)
\end{equation}

where $\alpha_k$ and $\beta_k$ are moment-matched parameters based on $E[\text{ASR}(k)]$ and $\sigma(k)$.

%-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------





\section{Bootstrap Trajectory Generation with Bayesian Posterior Sampling}
\label{appendix:bootstrap}

We model the uncertainty in attack success rates (ASR) using a principled Bayesian approach. For each behavior $i$, we assume there exists a true underlying probability $p_i$ of successfully triggering a safety violation on any given attempt.

\subsection{Prior Distribution}
We use a log-uniform prior distribution, which is appropriate for probabilities that may span multiple orders of magnitude. For a given range $[a, b]$, the probability density function is:

$$\pi(p) = \frac{1}{p \ln(b/a)}, \quad a \leq p \leq b$$

The prior bounds are determined from training data:
\begin{itemize}
    \item Upper bound $b = \max\{1/t_i\}$ where $t_i$ are observed first success times
    \item Lower bound $a = b e^{-w}$ where $w$ is a specified order of magnitude parameter
\end{itemize}

\subsection{Posterior Distribution for Uncensored Behaviors}
For behaviors where we observe a first success at time $t_i$, we derive the posterior distribution using Bayes' theorem. The likelihood of observing first success at time $t_i$ follows a geometric distribution:

$$L(t_i|p) = p(1-p)^{t_i-1}$$

Combined with our log-uniform prior, the posterior density is:

$$P(p|t_i) = \frac{t_i(1-p)^{t_i-1}}{\ln(b/a)[(1-a)^{t_i} - (1-b)^{t_i}]}, \quad a \leq p \leq b$$

This posterior naturally captures the uncertainty in our probability estimate, with the mode at $1/t_i$ and variance increasing with the waiting time.

\subsection{Handling Censored Behaviors}
For behaviors where no success is observed, we sample from a truncated version of the prior:

$$\pi_c(p) = \frac{1}{p \ln(a/c)}, \quad a \leq p \leq c$$

where $c = \min\{1/t_i\}$ is the minimum observed success probability. This ensures censored behaviors have lower probabilities than any observed success, reflecting our knowledge that these behaviors are more difficult to trigger.

\subsection{Sampling Algorithm}
For uncensored behaviors, we use rejection sampling to draw from the posterior:
\begin{enumerate}
    \item Propose $p$ from log-uniform distribution on $[a,b]$
    \item Accept with probability proportional to $(1-p)^{t_i-1}$
    \item Repeat until desired number of samples obtained
\end{enumerate}

For censored behaviors, we sample directly from the truncated log-uniform prior.

\subsection{Trajectory Generation}
For each sampled trajectory:
\begin{enumerate}
    \item Sample probabilities $p_i$ for each behavior:
        \begin{itemize}
            \item For uncensored: $p_i \sim P(p|t_i)$
            \item For censored: $p_i \sim \pi_c(p)$
        \end{itemize}
    \item Generate success/failure sequences: $X_{i,t} \sim \text{Bernoulli}(p_i)$
    \item Compute cumulative success indicator: $Y_i(t) = \mathbb{1}\{\exists s \leq t: X_{i,s} = 1\}$
    \item Calculate ASR: $\text{ASR}(t) = \frac{1}{N}\sum_{i=1}^N Y_i(t)$
\end{enumerate}

This approach provides a principled way to handle both observed and censored data while maintaining appropriate uncertainty estimates throughout the trajectory. The use of proper posterior distributions ensures that our uncertainty estimates accurately reflect both the timing of observed successes and the censoring of unsuccessful attempts.




% \section{Bootstrap Trajectory Generation with Log-Uniform Prior}
% \label{appendix:bootstrap}

% We model the uncertainty in attack success rates (ASR) using a principled Bayesian approach with log-uniform priors. For each behavior $i$, we assume there exists a true underlying probability $p_i$ of successfully triggering a safety violation on any given attempt.

% \subsection{Prior Distribution}
% We use a log-uniform prior distribution, which is appropriate for probabilities that may span multiple orders of magnitude. For a given range $[a, b]$, the probability density function is:

% $$\pi(p) = \frac{1}{p \ln(b/a)}, \quad a \leq p \leq b$$

% The prior bounds are determined from training data:
% \begin{itemize}
%     \item Upper bound $b = \max\{1/t_i\}$ where $t_i$ are observed first success times
%     \item Lower bound $a = b e^{-w}$ where $w$ is a specified order of magnitude parameter
% \end{itemize}

% \subsection{Handling Censored and Uncensored Behaviors}
% For each behavior $i$, we observe either a first success time $t_i$ or censoring (no success observed). We handle these cases differently:

% \paragraph{Uncensored Behaviors:} For behaviors where we observe a success at time $t_i$, we currently use a heuristic posterior distribution:
% $$\log p_i \sim \text{Uniform}(\log(1/t_i) - w/2, \log(1/t_i) + w/2)$$

% This maintains uncertainty around the observed probability while preserving the log-scale nature of the distribution. A more principled posterior derivation is left for future work.

% \paragraph{Censored Behaviors:} For behaviors where no success is observed, we sample from a truncated version of the prior:
% $$\log p_i \sim \text{Uniform}(\log(a), \log(c))$$
% where $c = \min\{1/t_i\}$ is the minimum observed success probability. This ensures censored behaviors have lower probabilities than any observed success.

% \subsection{Trajectory Generation}
% For each sampled trajectory:
% \begin{enumerate}
%     \item Sample probabilities $p_i$ for each behavior as described above
%     \item Generate success/failure sequences: $X_{i,t} \sim \text{Bernoulli}(p_i)$
%     \item Compute cumulative success indicator: $Y_i(t) = \mathbb{1}\{\exists s \leq t: X_{i,s} = 1\}$
%     \item Calculate ASR: $\text{ASR}(t) = \frac{1}{N}\sum_{i=1}^N Y_i(t)$
% \end{enumerate}

% Multiple trajectories are generated to estimate uncertainty bounds on the ASR curves. This approach provides a principled way to handle both observed and censored data while maintaining appropriate uncertainty estimates throughout the trajectory.

==> sections/5_power_laws_old.tex <==
% \section{Power Law Scaling}
% \label{sec:power_law_scaling}
% Given the strong performance of \BoN across modalities, we now explore fitting a mathematical model to the observed ASR, aiming to understand its scaling behavior. We find that negative log ASR exhibits power-law-like behavior and use it to forecast ASR with more samples.

% \subsection{Power Law Fitting}
% % The scaling behavior observed in \cref{fig:main_BoN_figure} (bottom) suggests a power-law-like relationship, with $-\text{log} (\text{ASR})$ as number of samples increases.
% The scaling behavior observed in \cref{fig:main_BoN_figure} (d), suggests we can fit a power law $-\text{log} (\text{ASR}) = a N^{-b}$ since the trend is linear in log-log space.
% % If this functional form fits our data well, it predicts that with enough samples, the ASR will asymptote to 100\%, effectively breaking all HarmBench queries.


% \begin{figure*}[h!]
%     \centering
%     \includegraphics[width=0.9\textwidth, trim=0.25cm 0.3cm 0.25cm 0.25cm]{figures/5_all_modalities_powerlaw.pdf}
%     \caption{\textbf{Negative log ASR exhibits power law-like behavior across models and modalities.} We fit each run of \BoN to $-\text{log}(\text{ASR}) = aN^{-b}$, using 7,200 steps (dashed lines) and compare to the bootstrapped error bars (shaded regions).}
%     \label{fig:all_modalities_powerlaws}
% \end{figure*}

% \paragraph{Experiment Details} To fit a power law to our data, we first transform the bootstrapped ASR trajectories by averaging, adding a small $\epsilon=1e-5$ in case of zero ASR and applying $y = -\log(\text{ASR})$. The model $\log(y) = a' - b \log(N)$ is fitted using linear regression with initialisation $a'=\log(3)$, $b=0.3$. We select logarithmically spaced $N$ when fitting the power law to avoid overweighting on densely populated data at larger $N$ and ignore the first five data points. Finally, $a'$ is exponentiated to revert to the power law form $y = aN^{-b}$, where $a = e^{a'}$ and $b$ reflects the decay parameter.



% \paragraph{Results} We find the power law fits the observed ASR across many models and modalities (\cref{fig:all_modalities_powerlaws}), aligning with work in scaling inference time compute \citep{snell2024scaling,chen2024more}. For many models, the slope (parameter $b$) is consistent, indicating a similar decay behavior across models. However, the intercept (parameter $a'$) varies significantly, showing that the scale factor driving ASR increase differs between models. Claude 3 Opus shows a much steeper slope, indicating that the ASR scales faster. Some models, such as GPT-4o (text), Claude 3 Opus (vision), and DiVA (audio), have regions of the expected ASR trajectory that are not linear, and the model shows signs better than power-law scaling. Other models show signs of plateauing for larger $N$, such as GPT-4o (audio).
% % However, even given deviations from perfect power-law scaling, the observed behavior is useful for forecasting.
% %We highlight that this power law equation does not include a constant as used in the power laws governing many-shot jailbreaking \cite{anil2024manyshotjailbreaking}. 


% % Since Llama 3 8B is jailbroken with 100\% ASR, we exclude it from \cref{fig:all_modalities_powerlaws} since the simple power law is inappropriate. 



% \subsection{Forecasting}
% % Given a functional form that fits the observed data, we can see if we can use it to forecast ASR even if some models don't show perfect power-law scaling. Forecasting allows us to predict the level of misuse risk for an LLM if an adversary has a much larger compute budget than we have.
% Given a functional form that fits the observed data, forecasting can help verify the validity of the power law. Additionally, it enables us to anticipate misuse risks for LLMs, particularly when adversaries leverage significantly larger compute budgets than ours.


% % This property is beneficial for practitioners looking to rapidly iterate with \BoN to identify optimal conditions for their dataset, knowing the achievable ASR with additional samples.

% % \paragraph{Bootstrapping with a prior} 
% % We found in forecasting experiments that using sampling without replacement as a bootstrapping procedure does not accurately extrapolate the data due to the tail of the bootstrapping estimates underestimating ASR.
% % When sampling without replacement, it does not account for requests that have not been jailbroken but may have been in a different independent run.
% % The inaccuracy of the tail end of bootstrapping can be seen in Fig.~\ref{fig:bootstrap_samples}. 



% \begin{wrapfigure}[20]{r}{0.49\textwidth}
%   \vspace{-1em}
%   \begin{center}
%     \includegraphics[width=0.9\linewidth, trim=0.25cm 0.25cm 0.25cm 0.25cm, clip]{figures/6_bootstrap_prior.pdf}
%   \end{center}
%   \caption{\textbf{Incorporating a probability distribution for jailbreak probability in bootstrapping ensures that trajectories from shorter runs are consistent with longer ones.} \texttt{Bootstrap-modified-short} generates trajectories that better follow \texttt{Bootstrap-long} and thus facilitate more accurate forecasting.}
%   \label{fig:bootstrap_prior}
% \end{wrapfigure}


% \paragraph{Experiment Details} To verify the power laws we find, we use the fitted power law to predict average ASR at large $N$ by extrapolating the behavior from smaller $N$. Our current bootstrapping procedure assumes that the probability of success is zero for the requests that never get jailbroken by the max $N$ we run. This assumption results in the bootstrapping estimate for larger $N$ underestimating ASR (\texttt{Bootstrap-short}; Fig.~\ref{fig:bootstrap_prior}). 
% To remedy this, we assign a probability distribution for requests not jailbroken by $N$ (implementation details in \cref{app:bootstrap-prior}; see \texttt{Bootstrap-modified-short} in Fig.~\ref{fig:bootstrap_prior}). We fit a power law to 100 trajectories generated with modified bootstrapping and use the standard deviation in prediction for error bars.





% \begin{figure*}[h!]
%     \centering
%     \includegraphics[width=0.9\textwidth, trim=0.25cm 0.3cm 0.25cm 0.25cm]{figures/7_forecasting_all_modalities.pdf}
%     \caption{\textbf{Power laws fit with only 1000 samples can forecast ASR within an order of magnitude more samples.} We fit each run of \BoN using a power law $-\text{log}(\text{ASR}) = aN^{-b}$ and extrapolate the ASR beyond the training data of 1000 samples, with error bars generated by fitting a power law to each bootstrapping trajectory. Our predictions have an error of 5.8\% averaged across models compared to the observed final ASR (marked with a cross).}
%     \label{fig:extrapolation_powerlaws}
% \end{figure*}

% \paragraph{Results} We find the fitted power laws can be used to forecast accurately over an order of magnitude. Specifically, in \cref{fig:extrapolation_powerlaws} (left), we predict the expected ASR on text models at $N=10,000$ having observed the expected ASR up to $N=1000$, and find we can extrapolate across an order of magnitude with errors of 1.1\%, 3.8\%, 0.2\% and 4.8\% on Sonnet, GPT-4o, Flash and Pro, respectively. We observe similar error rates for vision and audio when forecasting $N=7,200$ from $N=1000$. There is one exception for Gemini Pro vision, as we get an error of 18.5\% ASR---improvements in the probability distribution used in bootstrapping would help reduce this error rate, and we leave this for future work.

% Our results verify the observed power-law-like behavior is useful for forecasting with most models. Thus, it allows researchers to estimate how effective \BoN will be when increasing the sample size by an order of magnitude to understand the misuse risk with a higher compute budget.












% % \FloatBarrier


% % \begin{figure}[!h]
% %     \begin{minipage}{0.42\textwidth}
% %     \vspace{0pt}
% %     \paragraph{Experiment Details} To verify the power laws we find, we use the fitted power-law to predict average ASR at large $N$ by extrapolating the behavior from smaller $N$. Our current bootstrapping procedure assumes that the probability of success is zero for the requests that never get jailbroken by the max $N$ we run. This assumption results in the bootstrapping estimate for larger $N$ underestimating ASR (\texttt{Bootstrap-short}; Fig.~\ref{fig:bootstrap_prior}). 
% %     To remedy this, we assign a probability distribution for requests not jailbroken by $N$ (implementation details in \cref{app:bootstrap-prior}; see \texttt{Bootstrap-modified-short} in Fig.~\ref{fig:bootstrap_prior}). We use the mean of ASR trajectories generated by this modified bootstrap method to fit the power law.
    
% %         % \vspace{1em}
    
% %     \end{minipage}
% %     \hfill
% %     \begin{minipage}{0.53\textwidth}
% %     \vspace{0pt}
% %         \centering
% %         \includegraphics[width=0.9\linewidth]{figures/6_bootstrap_prior.pdf}
% %         \vspace{-0.5cm}
% %         \caption{\textbf{Incorporating a probability distribution for jailbreak probability in bootstrapping ensures that trajectories from shorter runs are consistent with longer ones.} \texttt{Bootstrap-modified-short} generates trajectories that better follow \texttt{Bootstrap-long} and thus facilitate more accurate forecasting.}
% %         \label{fig:bootstrap_prior}
% %     \end{minipage}
% % \end{figure}

% % \FloatBarrier




% % \paragraph{Bootstrapping with a prior} Our current bootstrapping procedure makes an assumption that the probability of success is zero for the requests that never get jailbroken. The result of this bad assumption is that the bootstrapping estimate for larger N underestimates the ASR (shown in Fig.~\ref{fig:bootstrap_samples}).
% % % We found in forecasting experiments that using sampling without replacement as a bootstrapping procedure does not accurately extrapolate the data due to the tail of the bootstrapping estimates underestimating ASR.
% % % When sampling without replacement, it does not account for requests that have not been jailbroken but may have been in a different independent run.
% % % The inaccuracy of the tail end of bootstrapping can be seen in Fig.~\ref{fig:bootstrap_samples}. 

% % To enhance the accuracy of our bootstrapping estimates in the tail, we incorporate a prior probability for the requests not jailbroken rather than assigning them a probability of zero. To do this, we calculate a probability of success for each request $p_i$ by using $p_i = \frac{1}{n_i}$, where $n_i$ is the number of samples needed for request $i$ to be successfully jailbroken. If we allow $p_i=0$ for all requests where a jailbreak is not observed in $N$ samples, we make the assumption that these requests will never be jailbroken regardless of how large $N$ gets . So instead, for each of these requests, we select a shift to the distribution $\hat{p}_i$ that is determined by sampling uniformly in log space between the minimum observed probability across all requests that are jailbroken within $N$ samples and a value five orders of magnitude lower. This is chosen by tuning on an independent GPT-4o-mini text run that makes the bootstrapping estimate equal to the ASR trajectory if more samples are run.

% % We generate many trajectories using the values of $p_i$ that incorporate the prior. The number of trials $n_i$ follows a geometric distribution truncated at $N$, with 
% % $$P(n_i = k) = p_i(1-p_i)^{k-1} \text{ for } k < N.$$



% % \begin{figure}[!h]
% %     \begin{minipage}{0.42\textwidth}
% %     \vspace{0pt}
    
% %     We generate $M$ bootstrap trajectories by sampling $n_i^{(m)} \sim \text{Geometric}(p_i)$ and estimate ASR at step $k \leq N$ over the total number of requests $R$ as
% %     $$\widehat{\text{ASR}}(k) = \frac{1}{M}\sum_{m=1}^M \left(\frac{1}{R}\sum_{i=1}^R \mathds{1}[n_i^{(m)} \leq k]\right)$$
    
% %     Figure~\ref{fig:bootstrap_prior} depicts bootstrapping estimates from a run with an early termination alongside a longer run, both with and without the implemented prior. This method empirically ensures that bootstrapping results from shorter runs are consistent with those from longer runs, facilitating more accurate forecasting.
        

% %         \vspace{1em}
    
% %     \end{minipage}
% %     \hfill
% %     \begin{minipage}{0.53\textwidth}
% %     \vspace{0pt}
% %         \centering
% %         \includegraphics[width=0.9\linewidth]{figures/6_bootstrap_prior.pdf}
% %         \vspace{-0.5cm}
% %         \caption{\textbf{The impact of incorporating a prior for the probability of success in bootstrapping.} The plot shows bootstrap traces from runs terminated early, demonstrating a more accurate estimation of a longer run when using a prior on the probability of success for each request.}
% %         \label{fig:bootstrap_prior}
% %     \end{minipage}
% % \end{figure}

% % \paragraph{Experiment Details} To verify the power laws we find, we use the fitted power-law to predict average ASR at large $N$ by extrapolating the behavior from smaller $N$. Utilizing bootstrapping with a prior, we use the mean of the ASR trajectories $\widehat{\text{ASR}}$ for fitting the power law and use the standard deviation of ASR across $M$ to plot the error bars.

==> shotgun_alg.tex <==
% \begin{algorithm}
% \caption{\BoN}
% \begin{algorithmic}[1]
% \Require Distribution $A$ for sampling augmentation vectors
% \Require Batch of requests $R = \{r_1, r_2 \ldots, r_n\}$
% \Require Target model $T$, classifier model $C$

% \While{$R \neq \emptyset$}
%     \State $a \sim A$ \Comment Sample augmentation i.i.d.
%     \State $R_{aug} \gets \{a(r) \mid r \in B\}$ \Comment{Apply augmentation to all prompts}
%     \For{$a(r_i) \in R_{aug}$}
%         \State $o_i \gets T(a(r_i))$ \Comment{Generate output for augmented prompt}
%         \If{$C(r_i, o_i) = 1$} \Comment{Classify output from target model}
%             \State $R \gets R \setminus \{r_i\}$ \Comment{Remove original prompt if jailbreak detected}
%         \EndIf
%     \EndFor
% \EndWhile
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}
\caption{\BoN}
\begin{algorithmic}[1]
\Require Distribution $A$ for sampling augmentation vectors
\Require Batch of requests $R = \{r_1, r_2 \ldots, r_n\}$
\Require Target model $T$, classifier model $C$
\Require Number of samples $N$

\For{$r_i \in R$}
    \For{$i \gets 1 \text{ to } N$}
        \State $a \sim A$ \Comment Sample augmentation i.i.d.
        \State $r_{i,aug} \gets a(r_i)$ \Comment{Apply augmentation to prompt $r_i$}
        \State $o_i \gets T(r_{i,aug})$ \Comment{Generate output for augmented prompt}
        \If{$C(r_i, o_i) = 1$} \Comment{Classify output from target model}
            \State \textbf{break} \Comment{Exit loop if jailbreak detected}
        \EndIf
    \EndFor
\EndFor
\end{algorithmic}
\label{alg:bon}
\end{algorithm}




==> tables/prepair_best_attacks.tex <==
% \begin{table}[h]
% \centering
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% \textbf{Model} & \textbf{Flash Text} & \textbf{Flash Audio} & \textbf{Pro Text} & \textbf{Pro Audio} \\
% \hline
% Highest Flash Audio & 15.09 & \textbf{76.73} & 9.43 & 33.96 \\
% Highest Flash Text & \textbf{37.74} & 25.16 & 0.63 & 0.00 \\
% Highest Pro Audio & 15.09 & 76.73 & 9.43 & \textbf{33.96} \\
% Highest Pro Text & 15.09 & 76.73 & \textbf{9.43} & 33.96 \\
% \hline
% \end{tabular}
% \caption{Highest ASR scores for each model and domain}
% \label{tab:highest_asr_scores}
% \end{table}

\begin{table}[h]
\centering
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Flash Text} & \textbf{Flash Audio} & \textbf{Pro Text} & \textbf{Pro Audio} \\
\midrule
Highest Flash Audio & 15.09 & \textbf{76.73} & 9.43 & 33.96 \\
Highest Flash Text & \textbf{37.74} & 25.16 & 0.63 & 0.00 \\
Highest Pro Audio & 15.09 & 76.73 & 9.43 & \textbf{33.96} \\
Highest Pro Text & 15.09 & 76.73 & \textbf{9.43} & 33.96 \\
\bottomrule
\end{tabular}
\caption{Highest ASR scores for each model and domain}
\label{tab:highest_asr_scores}
\end{table}


==> universal_jailbreak_asrs.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\textbf{Model} & Sonnet & Opus & 4o & Mini & Pro & Flash & Pro(A) & Flash(A)\\
\hline
\textbf{ASR} & 6.3\% & 34.6\% & 23.3\% & 23.9\% & 3.8\% & 17.6\% & XX & XX\\
\hline
\end{tabular}
}
\caption{\textbf{Initial ASRs on our test dataset for each of the prefixes we compose with BoN} \todo{get audio scores}}
\label{tab:universal_jailbreak_asrs}
\end{table}

